Beyond Visuals: Investigating Force Feedback in Extended Reality for Robot Data Collection

This work explores how force feedback affects various aspects of robot data collection within the Extended Reality (XR) setting. Force feedback has been proved to enhance the user experience in Extended Reality (XR) by providing contact-rich information. However, its impact on robot data collection has not received much attention in the robotics community. This paper addresses this shortcoming by conducting an extensive user study on the effects of force feedback during data collection in XR. We extended two XR-based robot control interfaces, Kinesthetic Teaching and Motion Controllers, with haptic feedback features. The user study is conducted using manipulation tasks ranging from simple pick-place to complex peg assemble, requiring precise operations. The evaluations show that force feedback enhances task performance and user experience, particularly in tasks requiring high-precision manipulation. These improvements vary depending on the robot control interface and task complexity. This paper provides new insights into how different factors influence the impact of force feedback.

==> Tables/result/objective_metrics/difference.tex <==
% \begin{table}[H]
% \centering
% \caption{P-values for difference of the objective metrics with and without force feedback.\\(*: p < 0.05 Significant difference, **: p < 0.01 Highly significant difference)}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{llcccc}
% \textbf{} & \textbf{Interface} & \textbf{Push Task} & \textbf{Pick Task} & \textbf{Assemble Task} & \textbf{Open Task} \\ \midrule
% {\textbf{Success Rate}} & MC-MCV & 0.154 & 1.000 & 0.011\textbf{*} & 0.154 \\
%                           & KT-KTF & 1.0 & 1.0 & 0.317 & 1.0 \\ \midrule


% {\textbf{Completion Time}} & MC-MCV & 0.338 & 0.560 & 0.001\textbf{**} & 0.186 \\
%                                & KT-KTF & 0.136 & 0.063 & 0.426 & 0.172 \\ \midrule

% \end{tabular}
% }

% \label{table:difference_object}
% \end{table}

% \begin{table}[H]
% \centering
% \caption{P-values for the difference in Success Rate with and without force feedback.\\($^*$: $p < 0.05$ Significant difference, $^{**}$: $p < 0.01$ Highly significant difference)}
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{l c c c c}
% \toprule
% \textbf{Interface} & \textbf{Push Task} & \textbf{Pick Task} & \textbf{Assemble Task} & \textbf{Open Task} \\ 
% \midrule
% MC-MCV & $0.154$ & $1.000$ & $\bm{0.011}^*$ & $0.154$ \\
% KT-KTF & $1.000$ & $1.000$ & $0.317$ & $1.000$ \\ 
% \bottomrule
% \end{tabular}
% }
% \label{table:success_rate}
% \end{table}

% \vspace{0pt} % Adjust spacing between tables

% \begin{table}[H]
% \centering
% \caption{P-values for the difference in Completion Time with and without force feedback.\\($^*$: $p < 0.05$ Significant difference, $^{**}$: $p < 0.01$ Highly significant difference)}
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{l c c c c}
% \toprule
% \textbf{Interface} & \textbf{Push Task} & \textbf{Pick Task} & \textbf{Assemble Task} & \textbf{Open Task} \\ 
% \midrule
% MC-MCV & $0.338$ & $0.560$ & $\mathbf{0.001}^{**}$ & $0.186$ \\
% KT-KTF & $0.136$ & $0.063$ & $0.426$ & $0.172$ \\ 
% \bottomrule
% \end{tabular}
% }
% \label{table:completion_time}
% \end{table}




==> Tables/result/objective_metrics/time.tex <==
\begin{table}[H]
\centering
\caption{Mean and standard deviation of completion time with and without force feedback.}
\begin{tabular}{l S[table-format=2.3]S[table-format=2.3]|S[table-format=2.3]S[table-format=2.3]|S[table-format=2.3]S[table-format=2.3]}
\toprule
\textbf{Interface} & \multicolumn{2}{c}{\textbf{Push Cube}} & \multicolumn{2}{c}{\textbf{Pick and Place}} & \multicolumn{2}{c}{\textbf{Assemble Peg}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& {Mean} & {SD} & {Mean} & {SD} & {Mean} & {SD} \\
\midrule
MC  & 36.039 & 14.262 & 27.172 & 11.894 & 45.542 & 16.448 \\
MCV & 33.770 & 10.772 & 21.919 &  9.645 & 29.828 & 15.815 \\
KT  & 17.662 &  7.682 & 17.180 &  8.483 & 18.231 &  9.487 \\
KTF & 15.118 &  6.420 & 13.427 &  5.268 & 16.156 &  5.788 \\
\bottomrule
\end{tabular}

\label{table:mean_time}
\end{table}


==> plots/success_rate.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{plots/image/success_rate.pdf}
    \caption{Success rate per task and interface.
    Each bar represents the success rate for a specific interface (MC, MCV, KT, KTF) across different tasks (Push, Pick, and Assemble).
    The success rates are shown as percentages, with values ranging from 0 to 100\%.}
    \label{fig:success_rate}
\end{figure}

==> plots/ueqs.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{plots/image/ueqs.pdf} % Change to your actual image filename
    \caption{
    Mean and standard error of UEQ-S questionnaire results for different interfaces. The introduction of force feedback enhances the overall user experience for both MC and KT. However, the improvement is more pronounced for the MC than for KT.
    }
    \label{fig:ueq_s_plot}
\end{figure}
